Resurrecting Submodularity for Neural Text Generation

Submodularity is desirable for a variety of objectives in content selection where the current neural encoder-decoder framework is inadequate. However, it has so far not been explored in the neural encoder-decoder system for text generation. In this work, we define diminishing attentions with submodular functions and in turn, prove the submodularity of the effective neural coverage. The greedy algorithm approximating the solution to the submodular maximization problem is not suited to attention score optimization in auto-regressive generation. Therefore instead of following how submodular function has been widely used, we propose a simplified yet principled solution. The resulting attention module offers an architecturally simple and empirically effective method to improve the coverage of neural text generation. We run experiments on three directed text generation tasks with different levels of recovering rate, across two modalities, three different neural model architectures and two training strategy variations. The results and analyses demonstrate that our method generalizes well across these settings, produces texts of good quality and outperforms state-of-the-art baselines.

==> trash.tex <==
On abstractive summarization, our method .
On MT, we obtain BLEU scores of 29.7 and 43.5 with Transformer \citep{scaling_nmt_ott2018scaling} on WMT'14 English-German and English-French tasks respectively, which to our knowledge is SoTA in the standard setup.\footnote{Standard setup means without pretrained models or extra monolingual data.}{On image-paragraph generation, our method achieves more than 2.5 improvements in CIDEr in both cross-entropy and self-critical training regimes \citep{melas-kyriazi-etal-2018-training} on the top-down model with CNN as encoder and LSTM as decoder with top-down attention \citep{top-down}.} Our source code will be available at \texttt{<redacted>}.

\begin{figure}[t!]
%\parbox{0.52\linewidth}{
%\vspace{-0.5em}
\begin{minipage}[t]{0.50\textwidth}
\setlength{\tabcolsep}{1.6pt}
\centering
\small
\captionof{table}{ROUGE F1 score and {MoverScore} (1-gram and 2-grams) results on CNN/DM.
}
\label{tab:cnn/dm}
% ${^\dag}$ denotes models retrained in our machine, ${^\P}$ denotes numbers reported from \citep{Liu2019TextSW}, and ${^\S}$ denotes the model obtained from the author.
%\vspace{0.7em}
%\toprule
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
        & \multicolumn{3}{c}{\textbf{ROUGE Scores}} 
        & \multicolumn{2}{c}{\textbf{MoverScore}} \\
        % & \multicolumn{1}{c}{\bf{Param}} \\
 \cmidrule(lr){2-4}   \cmidrule(lr){5-6}  
%  \cmidrule(lr){7-7}   
 \textbf{Model} &\bf{R-1} &\bf{R-2} &\bf{R-L} & \textbf{1-gr} & \textbf{2-gr}  \\
\midrule
LEAD-3                         & 40.00 & 17.50 & 36.28 & -- & --  \\
\midrule
\textbf{LSTM-based} \\ 
% \multicolumn{3}{l}{\textbf{PG-based models}}    \\ 
PG                    & 36.69  & 15.92 &  33.63  & 12.46 & 19.37  \\
PG +Cov.             & 39.08 & 17.09 & 35.92   & 17.55 &  24.17 \\
PG + Dim            & 40.01 & 17.74 & 36.94  & 17.56 &  24.16 \\
PG + DyDim & \textbf{40.13} & \bf{17.94} & \bf{37.21}  & \bf{17.77} & \bf{24.38} \\
\midrule
% Transformer    & 40.21 & 17.76  & 37.09 & -- & --  \\
% \midrule 
% % MASSBASE & 42.12 & 19.50 & 39.01 &  -- & --\\
% % BertSumExtAbs & 42.13 & 19.60 & 39.18 &  -- & -- \\
% UniLM & 43.33 & 20.21 & 40.51 &  -- & -- \\
% T5 & 43.52 & 21.55 & 40.69 &   -- & -- \\
\textbf{Large-Size Pretrained Models} \\ 
ERNIE-GEN & 44.02 & 21.17 & 41.26 &  -- & --\\
PEGASUS & 44.17 & 21.47 & 41.11 &  -- & -- \\
ProphetNet  & 44.20 & 21.17 & 41.30 &  -- & -- \\ 
BARTSum & 44.16 & 21.28 & 40.90 & 22.34 & 28.47 \\
   +Dim    & 44.86 & \bf{21.76} & 41.62 & 23.05 & 29.04  \\
   +DyDim  & \bf{44.92} & 21.70 & \bf{41.66} & \bf{23.12} & \bf{29.13} \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\setlength{\tabcolsep}{1.6pt}
\centering 
\small
\captionof{table}{ROUGE F1 score and {MoverScore} (1-gram and 2-gram) results on the NYT and XSum datasets. }
%\resizebox{\columnwidth}{!}{%
%        }
\end{minipage}
% \caption{ROUGE F1 score and \textbf{MoverScore} (1-gram and 2-grams) results on CNN/DM. ${^\dag}$ denotes that the models 
% {were retrained in our machine, ${^\P}$ denotes that numbers reported are from \citep{Liu2019TextSW}, and ${^\S}$ denotes that the pre-trained BSEA model was obtained from the author.}}
\label{table:sum-results}
%\end{table}
\vspace{-1em}
\end{figure}

        \midrule 
        \\[-0.6em]
        \textbf{XSum} & & & \\
        LEAD                      & 16.30 & 1.60 & 11.95 & -- & -- \\
        BertSum                    & 38.56 & 16.40 & 31.09  & 20.97 & 28.62  \\ 
        % \rowcolor{gray!15}
        + Dim              &  39.10 & 16.89 & 31.57  & 21.53 & 29.08 \\
        % \rowcolor{gray!15}
        + DyDim             & \textbf{39.18} & \textbf{16.97} & \textbf{31.62} & \textbf{21.75} & \textbf{29.34} \\
